Can Adversarial Examples Be Parsed to Reveal Victim Model Information?

Numerous adversarial attack methods have been developed to generate imperceptible image perturbations that can cause erroneous predictions of state-of-the-art machine learning (ML) models, in particular, deep neural networks (DNNs). Despite intense research on adversarial attacks, little effort was made to uncover 'arcana' carried in adversarial attacks. In this work, we ask whether it is possible to infer data-agnostic victim model (VM) information (i.e., characteristics of the ML model or DNN used to generate adversarial attacks) from data-specific adversarial instances. We call this 'model parsing of adversarial attacks' - a task to uncover 'arcana' in terms of the concealed VM information in attacks. We approach model parsing via supervised learning, which correctly assigns classes of VM's model attributes (in terms of architecture type, kernel size, activation function, and weight sparsity) to an attack instance generated from this VM. We collect a dataset of adversarial attacks across 7 attack types generated from 135 victim models (configured by 5 architecture types, 3 kernel size setups, 3 activation function types, and 3 weight sparsity ratios). We show that a simple, supervised model parsing network (MPN) is able to infer VM attributes from unseen adversarial attacks if their attack settings are consistent with the training setting (i.e., in-distribution generalization assessment). We also provide extensive experiments to justify the feasibility of VM parsing from adversarial attacks, and the influence of training and evaluation factors in the parsing performance (e.g., generalization challenge raised in out-of-distribution evaluation). We further demonstrate how the proposed MPN can be used to uncover the source VM attributes from transfer attacks, and shed light on a potential connection between model parsing and attack transferability.

==> secs/experiment.tex <==
\section{Experiments}
\label{sec: exp}
\subsection{Setup and implementation}
\paragraph{Dataset curation.} \YF{We first construct a set of victim models for each dataset (\textit{e.g.}, {\CIFAR}, {\CIFARM}, and {\TImageNet}). Besides robust-training models, all the other models are trained on the train set for 75 epochs using SGD optimizer with an initial learning rate of 0.1. The momentum and weight decay are set as 0.9 and 5e-4, respectively. The rewind epoch for sparse model training is set as 2. For robust-training models, XXX. Then, the dataset of attack features are generate for all the victim models. We split the test data of each ordinary dataset into two subsets. The first subset contains 80\% of the data and is used to generate attacks for {\MPN} and {\PEN} training, while the second subset is maintained to generate attacks for evaluation. We consider 7 attack generation methods with multiple different attack strength settings as shown in Table.\ref{tab: attacks}. Only the successfully attacked images are kept. }

\paragraph{{\MPN} training and evaluation.} 

\YF{To solve problem \eqref{eq: train_supervision}, we train {\MPN} using the SGD optimizer with an initial learning rate of 0.1. The training is conducted for 75 epochs with a batch size of 256 using cosine annealing learning rate schedule. For the joint optimization of {\MPN} and {\PEN} in problem \eqref{eq: pen_formulation}, we load a pretrained DnCNN from \cite{gong2022reverse} and fine-tune {\MPN} and {\PEN} jointly for XX epochs. The learning rate for {\MPN} and {\PEN} is set as 1e-3 and 1e-5, respectively. The regularization parameter $\beta$ is set as 1/15.  To evaluate the effectiveness of the proposed method, we evaluate both the in-distribution generalization and OOD generalization performance. }

\subsection{Results and insights} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{In-distribution performance for different {\AT} and attack methods.} \YF{We first show the in-distribution performance of model parsing for different attributes in \textbf{Table\,XXXX}. The experiments are conducted on the three datasets with different {\AT}. Each point shows the average individual attribute classification accuracy for the three attributes: {\KS}, {\AF}, and {\WS}. From the figure, we can see that {\MPN} can provide highly accurate attribution prediction with the input data format as perturbations, indicating surprisingly good generalization of {\MPN}. For example, model parsing with perturbations generated by {\PGD} can achieve almost 100\% in-distribution parsing accuracy in all shown scenarios. Meanwhile, though using adversarial images as input data format to {\MPN} can still reveal model attribute information (has an accuracy better than random guess), there is an obvious performance gap comparing to use perturbations. Then, we conduct an ablation study on the attack strength on {\CIFAR} with {\AT} as ResNet9, and the input data format is perturbations. The results are shown in \textbf{Fig. \ref{fig: mismatch_attack_strength}}, where the vertical axis represents the attack strength $\epsilon$ used for {\MPN} training while the horizontal axis indicates the $\epsilon$ used for testing. As can be seen from the figure, the main diagonal has the best model parsing performance as the train and test have the same attack strength. For off-diagonal cases, we can observe a performance degradation caused by attack strength mismatch. Furthermore, the closer the test time $\epsilon$ to the train time $\epsilon$, the higher model parsing accuracy can be achieved.  }  \YY{we need to have different attack types as x axis, avg parsing accuracies (given one attack method, across different attack strengths and attributes)  as y axis. Radar chart can be shown here. We list all attacks each with different strengths.} 

% \begin{figure}[htb]
% \centerline{
% \includegraphics[width=0.5\textwidth]{figs/in_dist_radar.png}
% }
% \caption{\footnotesize{\YY{A figure shows the consistent model parsing gap between adversarial examples  $\mathbf x^\prime$ and perturbations $\boldsymbol \delta$. For all $\ell_\infty$ attacks we choose $\epsilon = 8/255$; for all $\ell_2$ attacks we choose $\epsilon = 0.5$ except for {\CW} we choose $c=1$. Fix: only show one attack across different archs}
% }}
%  \vspace*{-1mm}
% \label{fig: x_prime_vs_delta}
% \end{figure}

\begin{table*}[htb]
    \centering
    \caption{\footnotesize{\YY{The in-distribution model parsing performance by different attack strength for each attack method measured by average attribute accuracy (\%) on {\CIFAR} and ResNet9. The $\ell_\infty$ norm is shown without $/255$.}}}
    \label{tab: in_distribution_all_strengths}
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{c || c | c | c | c | c | c | c |c | c | c| c | c | c | c | c | c | c |c | c | c|c | c | c | c | c | c | c | c |c | c | c| c | c | c | c | c | c | c |c  } 
    \toprule[1pt]
    \midrule
    \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Input}\\ \textbf{data}\end{tabular}}  & \multicolumn{39}{c}{\textbf{Attack methods}}  \\
    \cmidrule{2-40}
     % \cline{2-7}
      & \multicolumn{4}{c|}{{\FGSM}} & \multicolumn{4}{c|}{{\PGD} $\ell_\infty$} & \multicolumn{4}{c|}{{\PGD} $\ell_2$} & \multicolumn{3}{c|}{\CW}  & \multicolumn{4}{c|}{{\AutoAttackShort} $\ell_\infty$} & \multicolumn{4}{c|}{{\AutoAttackShort} $\ell_2$} & \multicolumn{4}{c|}{{\SquareAttackShort}  $\ell_\infty$} &\multicolumn{4}{c|}{{\SquareAttackShort}  $\ell_2$} & \multicolumn{4}{c|}{\NES} & \multicolumn{4}{c}{\ZOSignSGD} \\
\cmidrule{2-40}
  &4&8&12&16&4&8&12&16&0.25&0.5&0.75&1&0.1&1&10 &4&8&12&16&0.25&0.5&0.75&1&4&8&12&16&0.25&0.5&0.75&1&4&8&12&16&4&8&12&16 \\
    \midrule
    $\mathbf{x}^\prime$ & 60      &78     &86     &90     &50     &66     &76     &75     &36     &53     &62     &71     &33     &35     &36     &58     &74     &82     &86     &38     &56     &66     &78     &35     &38     &39     &39     &37     &36     &36     &36     &35     &40     &42     &41     &35     &42      &44     &44         \\
    $\bdelta_{\PEN}$ & 85      &94     &95     &96     &76     &83     &89     &86     &62     &82     &89     &91     &55     &64     &64     &84     &91     &93     &94     &66     &86     &93     &96     &44     &44     &43     &42     &38     &42     &41     &40     &52     &58     &60     &59     &55     &61      &62     &62       \\
    $\bdelta$   & 96      &96     &96     &96     &96     &95     &94     &91     &99     &99     &99     &99     &96     &96     &96     &97     &97     &97     &96     &99     &99     &99     &99     &46     &44     &42     &42     &44     &44     &43     &41     &79     &83     &83     &83     &81     &84      &85     &85             \\
    \midrule
    \bottomrule[1pt]
    \end{tabular}}
\end{table*}


\begin{table*}[htb]
\centering
\caption{\footnotesize{\YY{The in-distribution model parsing performance by different attack strength for each dataset and victim model pair measured by average attribute accuracy (\%). The $\ell_\infty$ norm is shown without $/255$.}}}
    \label{tab: in_distribution_arch_all_strengths}
\resizebox{\textwidth}{!}{
\begin{tabular}{cc||ccc|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule[1pt]\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Attack}\\\textbf{ methods}\end{tabular}} & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}} $\epsilon$ \\ or\\ $c$ \end{tabular}}& \multicolumn{18}{c}{\textbf{Dataset and victim model}} \\ \cmidrule{3-23} 
 & &\multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}{\CIFAR}\\ ResNet9\end{tabular}}&\multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}{\CIFAR}\\ ResNet18\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}{\CIFAR}\\ ResNet20\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}{\CIFAR}\\ VGG11\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}{\CIFAR}\\ VGG13\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}{\CIFARM}\\ ResNet9\end{tabular}} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}{\TImageNet}\\ ResNet18\end{tabular}} \\ \cmidrule{3-23} 
 & &\multicolumn{1}{c|}{$\mathbf {x}^\prime$} & \multicolumn{1}{c|}{$\bdelta_\mathrm{PEN}$} & \multicolumn{1}{c|}{$\bdelta$}  & \multicolumn{1}{c|}{$\mathbf {x}^\prime$} & \multicolumn{1}{c|}{$\bdelta_\mathrm{PEN}$} & \multicolumn{1}{c|}{$\bdelta$} & \multicolumn{1}{c|}{$\mathbf {x}^\prime$} & \multicolumn{1}{c|}{$\bdelta_\mathrm{PEN}$} & \multicolumn{1}{c|}{$\bdelta$} & \multicolumn{1}{c|}{$\mathbf {x}^\prime$} & \multicolumn{1}{c|}{$\bdelta_\mathrm{PEN}$} & \multicolumn{1}{c|}{$\bdelta$} & \multicolumn{1}{c|}{$\mathbf {x}^\prime$} & \multicolumn{1}{c|}{$\bdelta_\mathrm{PEN}$} & \multicolumn{1}{c|}{$\bdelta$} & \multicolumn{1}{c|}{$\mathbf {x}^\prime$} & \multicolumn{1}{c|}{$\bdelta_\mathrm{PEN}$} & \multicolumn{1}{c|}{$\bdelta$} & \multicolumn{1}{c|}{$\mathbf {x}^\prime$} & \multicolumn{1}{c|}{$\bdelta_\mathrm{PEN}$} & \multicolumn{1}{c}{$\bdelta$} \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}{\FGSM}\end{tabular}} 
&0.25&  60.13   &85.25  &96.82  &60.0   &86.92  &97.66  &62.41  &88.91  &97.64  &47.42  &-1.0   &91.75  &66.28  &-1.0   &98.57  &57.99  &-1.0   &94.86  &37.23  &-1.0   &97.04  \\
&0.5& 78.8    &94.15  &96.89  &80.44  &95.49  &97.61  &82.29  &95.9   &97.72  &63.13  &-1.0   &92.41  &84.92  &-1.0   &98.66  &75.58  &-1.0   &94.96  &70.29  &-1.0   &97.05 \\
&0.75&86.49   &95.96  &96.94  &88.03  &96.89  &97.68  &88.71  &97.13  &97.81  &73.71  &90.19  &92.66  &91.21  &-1.0   &98.71  &82.27  &-1.0   &95.55  &76.0   &-1.0   &97.02 \\
&1&90.16   &96.43  &96.94  &91.71  &97.34  &97.68  &91.84  &97.47  &97.79  &79.51  &-1.0   &92.6   &94.22  &-1.0   &98.73  &86.5   &-1.0   &94.74  &79.63  &-1.0   &96.87 \\
\midrule
\multirow{4}{*}{{\PGD} $\ell_\infty$} 
&4& 50.54   &76.43  &96.02  &56.94  &79.45  &96.96  &55.01  &80.05  &97.49  &39.33  &66.38  &91.84  &57.12  &-1.0   &98.29  &42.27  &-1.0   &92.65  &35.48  &-1.0   &97.18\\
&8&66.62   &83.2   &95.07  &73.29  &87.29  &95.38  &67.49  &86.19  &96.18  &56.62  &81.14  &92.78  &69.16  &-1.0   &97.22  &59.71  &-1.0   &90.43  &61.85  &-1.0   &96.05 \\
&12&76.65   &89.73  &94.91  &81.73  &91.67  &95.55  &76.41  &90.16  &95.67  &70.56  &88.92  &94.13  &78.67  &-1.0   &97.26  &70.86  &-1.0   &91.28  &73.82  &-1.0   &96.38   \\
&16&  75.58   &86.95  &91.28  &82.46  &90.19  &93.19  &76.58  &87.79  &92.5   &72.13  &87.23  &91.85  &78.28  &-1.0   &94.66  &71.29  &-1.0   &86.84  &73.19  &-1.0   &93.54   \\
\midrule
\multirow{4}{*}{{\PGD} $\ell_2$} 
&0.25& 36.75   &62.2   &99.66  &46.35  &70.17  &99.74  &48.24  &77.22  &99.75  &36.47  &45.17  &98.52  &35.81  &-1.0   &99.85  &35.92  &-1.0   &99.29  &35.55  &-1.0   &99.68   \\
&0.5& 53.42   &82.58  &99.64  &60.89  &84.7   &99.56  &61.62  &89.11  &99.61  &41.56  &66.58  &98.68  &57.83  &-1.0   &99.83  &48.89  &-1.0   &99.01  &35.52  &-1.0   &99.71  \\
&0.75& 62.66   &89.04  &99.48  &71.01  &89.89  &99.22  &70.76  &92.06  &99.36  &47.02  &-1.0   &98.52  &72.76  &-1.0   &99.74  &59.19  &-1.0   &98.61  &35.56  &-1.0   &99.71   \\
&1&  71.65   &91.73  &99.26  &77.09  &92.09  &98.94  &76.84  &92.82  &98.96  &54.2   &-1.0   &98.41  &79.93  &-1.0   &99.57  &66.97  &-1.0   &97.89  &43.48  &-1.0   &99.64   \\
\midrule
\multirow{3}{*}{\CW} 
&0.1& 33.77   &55.6   &96.71  &47.77  &63.26  &96.11  &33.56  &63.11  &94.1   &33.73  &-1.0   &94.37  &33.68  &-1.0   &96.95  &34.41  &-1.0   &92.55  &35.96  &-1.0   &95.52   \\
&1& 35.42   &64.46  &96.66  &45.75  &65.25  &97.45  &33.74  &62.71  &97.08  &33.89  &-1.0   &91.29  &36.12  &-1.0   &98.58  &34.25  &-1.0   &93.25  &35.54  &-1.0   &89.35  \\
&10& 36.38   &64.45  &96.64  &45.83  &65.32  &97.41  &33.83  &63.52  &97.11  &38.29  &-1.0   &91.33  &38.51  &-1.0   &98.62  &34.25  &-1.0   &93.18  &35.45  &-1.0   &94.2   \\\midrule\bottomrule[1pt]
\end{tabular}}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Effectiveness encountering mismatched attack strengths. } Fig.\,\ref{fig: mismatch_attack_strength} \YY{shows the model parsing performance degradation by mismatched attack strengths on different attack types on {\CIFAR} when {\AT} is ResNet9.}

\begin{figure}[htb]
\centerline{
\includegraphics[width=0.5\textwidth]{figs/diff_strength.png}
}
\caption{\footnotesize{\YY{A figure shows the degradation brought by the mismatched attack strength when taking $\bdelta$ as input.}
}}
 \vspace*{-1mm}
\label{fig: mismatch_attack_strength}
\end{figure}

% \begin{table}[htb]
%     \centering
%     \caption{\footnotesize{\YY{The in-distribution model parsing performance by grouping different attack strengths for each attack method measured by average attribute accuracy (\%) on {\CIFAR} and ResNet9.}}}
%     \label{tab: group_attack_strength}
%     \resizebox{0.47\textwidth}{!}{
%     \begin{tabular}{c || c | c | c | c | c | c | c |c | c | c} 
%     \toprule[1pt]
%     \midrule
%     \textbf{Input}  & \multicolumn{10}{c}{\textbf{Attack methods}}  \\
%      \cmidrule{2-11}
%      % \cline{2-11}
%     \textbf{data}   & {\FGSM} & {\PGD} $\ell_\infty$ & {\PGD} $\ell_2$ & \CW  & {\AutoAttackShort} $\ell_\infty$ & {\AutoAttackShort} $\ell_2$ & {\SquareAttackShort}  $\ell_\infty$ &{\SquareAttackShort}  $\ell_2$ & \NES & \ZOSignSGD \\
%     \midrule
%     $\mathbf{x}^\prime$ & 81.20    &70.94  &60.16  &38.89  &80.54  &65.40   &40.33  &36.50   &40.01  &44.37    \\
%     $\bdelta_{\PEN}$    & 94.85   &87.38  &86.36  &64.32  &93.13  &90.23  &45.00   &42.96  &61.90   &64.33    \\
%     $\bdelta$           & 97.70    &95.95  &99.75  &96.99  &98.51  &99.97  &45.78  &45.99  &85.42  &89.11    \\
%     \midrule
%     \bottomrule[1pt]
%     \end{tabular}}
% \end{table}

\begin{table}[htb]
    \centering
    \caption{\footnotesize{\YY{The in-distribution model parsing performance by grouping different attack strengths for each attack method measured by average attribute accuracy (\%) on {\CIFAR} and ResNet9.}}}
    \label{tab: group_attack_strength}
    \resizebox{0.47\textwidth}{!}{
    \begin{tabular}{c | c | c | c | c | c | c | c |c | c | c} 
    \toprule[1pt]
    % \midrule
\diagbox{Input data}{Attack type} & {\FGSM} & \begin{tabular}[c]{@{}c@{}}     
      {\PGD} \\ 
      $\ell_\infty$
      \end{tabular}
      & 
      \begin{tabular}[c]{@{}c@{}}     
      {\PGD} \\ 
      $\ell_2$
      \end{tabular} 
      & {\CW} & 
      \begin{tabular}[c]{@{}c@{}}     
      {\AutoAttackShort} \\ 
      $\ell_\infty$
      \end{tabular} & 
    \begin{tabular}[c]{@{}c@{}}     
      {\AutoAttackShort} \\ 
      $\ell_2$
      \end{tabular}
      & {\NES} &  \begin{tabular}[c]{@{}c@{}}     
      {\texttt{ZO}-} \\ 
      {\texttt{signSGD}}
      \end{tabular} & \begin{tabular}[c]{@{}c@{}}     
      {\SquareAttackShort} \\ 
      $\ell_\infty$
      \end{tabular} & 
\begin{tabular}[c]{@{}c@{}}     
      {\SquareAttackShort} \\ 
      $\ell_2$
      \end{tabular}\\
    \midrule
    $\mathbf{x}^\prime$ & 81.20    &70.94  &60.16  &38.89  &80.54  &65.40   &40.01  &44.37 &40.33  &36.50      \\ \midrule
    $\bdelta_{\PEN}$    & 94.85   &87.38  &86.36  &64.32  &93.13  &90.23   &61.90   &64.33 &45.00   &42.96     \\ \midrule
    $\bdelta$           & 97.70    &95.95  &99.75  &96.99  &98.51  &99.97  &85.42  &89.11  &45.78  &45.99    \\ 
    % \midrule
    \bottomrule[1pt]
    \end{tabular}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{OOD generalization of {\MPN}} \YF{As there could exist attack/model distribution shifts in $\mathcal D_\mathrm{test}$, We further test the OOD generalization of {\MPN} for both attack distribution shift and model distribution shift case. For attack distribution shifts, we conduct experiments on {\CIFAR}, ResNet9 with different attack methods $\mathcal A$, and the results are shown in \textbf{Fig. \ref{fig: id_vs_ood}}. The vertical axis stands for the attack methods used for training, and the horizontal axis is the evaluation attack methods. The brighter implies a better generalization ability. From the figure, we can see that if the unseen attack is similar to the attack method used for training, {\MPN} can provide good generalization performance.  However, the generalization of {\MPN} becomes difficult for unseen attacks dissimilar to the train time attacks. Take the second row as an example, {\MPN} trained on {\FGSM} still has good generalization with an average accuracy higher than 80\% for {\PGD} and {\AutoAttackShort}, but the accuracy for other attack methods is less than 40\% }

\begin{figure}[htb]
\centerline{
\includegraphics[width=0.48\textwidth]{figs/ood.png}
}
\caption{\footnotesize{\YY{A figure shows the id and OOD performance of MPN on different attack methods on {\CIFAR}, ResNet9 given $\bdelta$ as input. For all $\ell_\infty$ attacks we choose $\epsilon = 8/255$; for all $\ell_2$ attacks we choose $\epsilon = 0.5$ except for {\CW} we choose $c=1$.}
}}
 \vspace*{-1mm}
\label{fig: id_vs_ood}
\end{figure}

\YY{Fig.\,\ref{fig: id_vs_ood} shows five blocks of different attack methods studied, \textit{i.e.,} $\ell_\infty$ WB, {\CW}, $\ell_2$ WB, query-based BB, and random serach BB. Based on the Table\,\ref{tab: group_attack_strength} and Fig.\,\ref{fig: id_vs_ood}, we choose {\PGD} $\ell_\infty$, {\PGD} $\ell_2$, {\CW}, and {\ZOSignSGD} as a mixed attack method training dataset including different choices of attack strengths to ensure the model parsing performance on different attack methods. }


\begin{figure}[htb]
\centerline{
\includegraphics[width=0.5\textwidth]{figs/selected_attacks.png}
}
\caption{\footnotesize{\YY{This figure should be compared with any single attack trained model parser performance. A fix solution for different attack methods on CIFAR-10 ResNet9. We choose {\PGD} $\ell_\infty$, {\PGD} $\ell_2$, {\CW}, and {\ZOSignSGD} as a mixed attack method training dataset including all different choices of attack strengths to ensure the model parsing performance on different attack methods.}
}}
 \vspace*{-1mm}
\label{fig: fix_solution}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\YF{Similarly, we conduct experiments on model distribution shift case, and the results are shown in \textbf{ Fig. \ref{fig: diff_arch}}.  }
\paragraph{Model parsing results on different architectures given one attack method.} Fig.\,\ref{fig: diff_arch}.

\begin{figure}[htb]
\centerline{\includegraphics[width=0.5\textwidth]{figs/diff_arch.png}}
\caption{\footnotesize{\YY{Different {\AT} is hard to parse even if $\bdelta$ is given as input. Another line of fix-solution figure should include some selected architectures to show the improvement.}}}
\label{fig: diff_arch}
\end{figure}


\YF{Combining the results in Fig. \ref{fig: id_vs_ood}, to obtain a {\MPN} with good generalization ability for different attack methods, we consider using data augmentations during training by feeding {\MPN} with several distinct attack methods. }

\paragraph{Effectiveness grouping different attack strengths. } Fig.\,\ref{tab: group_attack_strength} \YY{shows the model parsing performance by grouping different attack strengths for each attack method respectively on {\CIFAR} when {\AT} is ResNet9.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{{\AT} classification effectiveness.} Fig.\,\ref{fig: arch_class} \YY{shows the model parsing performance with {\AT} merged}

\begin{figure}[htb]
\centerline{
\includegraphics[width=0.5\textwidth]{figs/4attr.png}
}
\caption{\footnotesize{\YY{In-distribution performance including 4 attributes. A figure shows the effectiveness when {\AT} is merged. Each attack method is corresponding to an attribute classification including 5 {\AT}, 3 {\KS}, 3 {\AF}, and 3 {\WS}. The weighted average accuracy is reported on {\CIFAR} and ResNet9}  
}}
\label{fig: arch_class} 
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{The visualization by TSNE plot.} Fig.\,\ref{fig: tsne} 
% \YY{given a victim model architecture, we can visualize the feature embeddings of different attribute combinations by {\MPN}.}

% \begin{figure}[htb]
% \centerline{
% \includegraphics[width=0.5\textwidth]{figs/tsne.pdf}
% }
% \caption{\footnotesize{\YY{A figure shows the distinction between features of MPN. Different {\AT} and {\KS} can be differentiated really well while {\WS} is harder to cluster given the other attributes the same. The architecture is ResNet9 and the dataset is {\CIFAR}.}  
% % \JC{TODO: feature map}
% }}
%  \vspace*{-1mm}
% \label{fig: tsne}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Overall model parsing results on different attacks.} Fig.\,\ref{fig: id_vs_ood} 
\YY{we need to cross different attack types and evaluate the model parsing results. From this overall figure, we can see that the strong model parsing ability across similar attack methods.}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The model parser reveals the real victim.} Fig.\,\ref{fig: transfer_attack} 
\YY{Can we reveal the victim model (substitude model) on which the transfer attack was generated?}

\begin{figure}[htb]
\centerline{
\includegraphics[width=0.5\textwidth]{figs/transfer_corr.png}
}
\caption{\footnotesize{\YY{Scatterplot to show that the model parser can reveal the real victim (blue)(\textit{i.e.}, the source model) instead of the transfer attack's target model (orange).} %\JC{TODO: Transfer attacks}
}}
 \vspace*{-1mm}
\label{fig: transfer_attack}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The connection between model parsing and transfer attack successful rate.} Fig.\,\ref{fig: parsing_vs_transfer} 
\YY{If there are any attribute settings easily to be confused by the model parser, will the corresponding models' adversarial examples easily transfer to each other?}

% \begin{figure}[htb]
% \centerline{
% \includegraphics[width=0.5\textwidth]{figs/parsing_vs_transfer.png}
% }
% \caption{\footnotesize{\YY{One pair of images to show the correlation between model parsing and transfer attack successful rates}
% }}
%  \vspace*{-1mm}
% \label{fig: parsing_vs_transfer}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The model parsing ability for unseen \AT.} Fig.\,\ref{fig: unseen_at} 
\YY{If the model parser is trained on selected archtectures and tested on the other, what will be the performance?}

\begin{figure}[htb]
\centerline{
\includegraphics[width=0.5\textwidth]{figs/unseen_at.png}
}
\caption{\footnotesize{\YY{TODO: Partial archs. Model parsing ability towards unseen \AT.} \JC{TODO}
}}
 \vspace*{-1mm}
\label{fig: unseen_at}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The model parsing ability for adversarially robust models.} Fig.\,\ref{fig: robust_parsing} 
\YY{Given an adversarailly robust victim model, the model parser performance would be degraded.}

\begin{figure}[htb]
\centerline{
\includegraphics[width=0.5\textwidth]{figs/parse_adv_model.png}
}
\caption{\footnotesize{\YY{Model parsing over robust models' adversarial examples is difficult. There are four blocks in the heat map: the upper left one indicates the good model parsing performance over standard trained models while the lower right one indicates the difficulty of parsing adversarial examples against robust models.}
}}
 \vspace*{-1mm}
\label{fig: robust_parsing}
\end{figure}



==> secs/introduction.tex <==
\section{Introduction}

\paragraph{What is the reverse engineering of deceptions (RED)?} Introduce the concept of RED and differentiate it from adversarial defenses including adversarial detections and adversarial robustness.

\paragraph{What are prior works of RED?} Introduce what has been done in the field of RED. We should include the most relevant in the introduction, such as RED of adversarial perturbations \cite{gong2022reverse}, adversarial attack types \cite{oh2019towards} \YY{TODO: Add more refs}. \YY{[Feel free to check related work  (google sheets) and learn how they organize their papers and sell their stories.]} We should mention the GAN-based model parsing to motivate single adversarial example-based fine-grained model parsing, including activation function, kernel size, and pruning scheme, \textit{etc.}.

\paragraph{The feasibility of model parsing} We should state the adversarial attack generation is strongly correlated with model information. That's why we can implement model parsing functions over a single adversarial example. Here we can show one figure including the model parsing effectiveness similar to Figure 1 of \cite{souri2021identification}.

\paragraph{What are the challenges?} Although adversarial perturbations can help us apply model parsing, there exists a gap between adversarial images and perturbations. At the same time, due to the distribution shifts between different attack methods and different model architectures, we should consider how to achieve unseen attack-based model parsing and correlate the unseen model architecture with the nearest neighbor in the existing attack library.


\begin{figure}
\centering
  \includegraphics[width=0.5\textwidth]{figs/overview.png}%
  \caption{\footnotesize{Overview of model parsing by adversarial images.}}
\end{figure}

\paragraph{Our proposed method.} We propose a model-parsing objective enhanced denoiser (\YY{An overview of the pipeline should be shown here.}) to close the gap between adversarial images and perturbations. We conduct extensive experiments to show the effectiveness of adversarial example-based model parsing across different attack types, different attack strengths, and victim model architectures.

\paragraph{The key factors of model parsing.} According to the experimental results, we find 

1) model parsers have better generalization over gradient-based attacks with similar attack strengths (epsilons). 

2) model parsers trained on weaker attack yields better out-of-distribution generalization over stronger attack. 

3) black-box attacks are more difficult to model parse than white-box attacks considering victim model dependency. 

4) Transfer attacks will reveal their originally attacked surrogate model information instead of the target victim model. As for transfer attack, we need one figure to show the effectiveness of our parser to reveal the real victim instead of the target.

5) Robust models' adversarial examples are harder to model parse due to the distribution of perturbations.

6) RED performance versus the attack transferability. The easier one attribute is to apply a transfer attack, the harder it is model parsed, e.g., sparse models' attack can easily transfer to dense models.

7) The model parsing precision (confidence) towards different model architectures correlates with the model's generalization and robustness.

\paragraph{Concluding the key factors we summon up one dataset to train the model parser.}

\paragraph{Our contributions.} In this paper,

1) We find the feasibility of adversarial perturbations to solve the model parsing problem;

2) We propose a denoiser-based model parsing method to close the gap between adversarial images and perturbations;

3) We conduct extensive experiments to show our method's model parsing ability and key factors that influence the model parsing. 





==> secs/method.tex <==
\section{Method}
Though adversarial images can reveal victim model information, there is a clear performance gap between using adversarial images and the adversarial perturbation $\boldsymbol \delta$. As the groundtruth $\boldsymbol \delta$ is hard to obtain, it is necessary to consider how to bridge the gap.    

% In this section, we should clearly state how we formulate a model-parsing-enabled perturbation extraction pipeline. We can mimic our ICLR2022 paper or the denoised-smoothing paper by Zico Kolter.


==> secs/motivation.tex <==
\section{Motivation}
\paragraph{Rationale of adversarial attack generation.} The rationale behind the model parsing by adversarial examples is supported by the model dependency when generating adversarial perturbations. As for white-box attacks, such as PGD, FGSM, and CW attacks, \textit{etc.}, each attack generation iteration is strongly correlated with the model gradients.



% Tab.\,\ref{tab: attack_vs_model} shows the potential of model parsing by adversarial examples. 

\paragraph{Formualtion of model parsing} Motivated by the attack generation dependency over model information, we formulate our model parsing problem as: \YY{TODO: an optimization formulation}

\paragraph{Warm-up examples: adversarial perturbations are all you need} We should have a big matrix to show the in-distribution model parsing ability by adversarial perturbations. 

\paragraph{Gap between images and perturbations}



==> secs/outline_YY.tex <==

\begin{center}
    \textbf{Outline of the paper}
\end{center}

\YY{[Feel free to check related work  (\href{https://docs.google.com/spreadsheets/d/1RQf5lhpShi4cgaUKUxsCLYkYY8meRq_Igi0Sq_2okq8/edit?usp=sharing}{[selected list]} and beyond) and learn how they organize their papers and sell their stories.]}

\begin{enumerate}
    \item \textbf{Introduction.}  Considering to include the following paragraphs/topics
    \begin{enumerate}
        \item What is reverse engineering of deceptions (\textbf{RED}) and why it?
        \SL{[You need differentiate RED and Model Parsing. Let us focus on Model Parsing, a challenging RED task.]}
        \item Predominant RED applications, methods, and challenges: what kind of attributes do the prior works focus on? How do they solve it? What is missing? 
        \item Briefly review the most relevant works about RED (Examples: our ICLR RED work, attack attribution work \cite{souri2021identification} ) and state our \textbf{contributions}.
            
        \textbf{Remark:} We need a \textbf{Figure} in the Introduction to show the RED pipeline and the most significant experiment results (possibly together with the key technology).
        Examples: our ICML23 unlearning paper.
    \end{enumerate}
        \item \textbf{Related work}
        \begin{enumerate}
        \item RED
        \item NAS vs Robustness (\href{https://docs.google.com/spreadsheets/d/1RQf5lhpShi4cgaUKUxsCLYkYY8meRq_Igi0Sq_2okq8/edit#gid=0}{link})
    \end{enumerate}

    \item \textbf{Problem Statement}.
    \begin{enumerate}
        \item A primer on RED
        \item Problem of interest: Model parsing. 
        \textbf{Key} is to define and collect `\textbf{model attributes}'.
    \end{enumerate}

    \item \textbf{Main technical sections: Including warm-ups and methods.}

    \item \textbf{Experiments}

\begin{enumerate}
    \item Experiment setup. One example is \href{https://openreview.net/pdf?id=MjsDeTcDEy}{Sec.\,6.1}.
    \begin{enumerate}
        \item Datasets, models, and attack methods.
        \item Implementations.
        \item Training and evaluation setups.
    \end{enumerate}
    \item Experiment results. Focusing on results complements to the previous sections. One example is \href{https://openreview.net/pdf?id=MjsDeTcDEy}{Sec.\,6.2} or \href{https://arxiv.org/pdf/2211.11635.pdf}{Sec.\,V-B}.

    \item \textbf{Experiment cluster 1}: \textbf{Is it possible to achieve (victim) model parsing from adversarial attacks?} 

    \begin{enumerate}
        \item \textbf{Exp1.1}: Fix a dataset and consider two types of inputs, $\bdelta$ (adversarial perturbations) and $\mathbf x^\prime$ (adversarial examples); please show the feasibility of model parsing and the advantage of $\bdelta$  over $\mathbf x^\prime$?
        \begin{enumerate}
            \item When evaluating performance of \textbf{Exp1.1}, please consider both in-distribution assessment and out-of-distribution assessment. In the context of PGD, you could determine this via train-time attack radius vs. test-time attack radius. 
        \end{enumerate}
        \item \textbf{Exp1.2}: Extend Exp1.1 over \textbf{diverse attack methods}. E.g., the training set and testing set  include multiple attack types, such as FGSM, PGD linf, PGD l2, CW, AuotAttack, Black-box Attack.
        \item \textbf{Exp1.3}: Extend Exp1.1 over \textbf{diverse datasets} (especially for those with different input resolutions, MNIST, CIFAR-10, Tiny-ImageNet). 
\item  \textbf{Goal of Exp1}: Showing the feasibility of model parsing for adversarial attacks as a \textbf{generic finding}. 
\SL{Matrix presentation? \href{https://arxiv.org/pdf/1802.04434.pdf}{Fig. A2} or \href{https://arxiv.org/pdf/1908.08016.pdf}{Fig. 4}.}
    \end{enumerate}

    \item \textbf{Experiment cluster 2}: \textbf{How to reduce the gap between model parsing using $\boldsymbol \delta$ and model parsing using $\mathbf x^\prime$?}

    \begin{enumerate}
        % \item  \textbf{Exp2.1} Try the \href{https://github.com/MotasemAlfarra/Combating-Adversaries-with-Anti-Adversaries}{anti-adversary} method to estimate $\delta$. 
        \item \textbf{Exp2.1}  Try the proposed model parsing-aware estimation method in this paper.
        \[
        \min_{\phi, \theta}L_{\mathrm{CE}}(f_\theta(x^\prime - D_\phi(x^\prime)),y)  + L_{\mathrm{MAE}}((D_\phi(x^\prime)),x)
        \]
        \item Based on the above, evaluation following Exp.1. 
    \end{enumerate}


    \item \textbf{Experiment cluster 3}: \textbf{Can we achieve model parsing about the black-box victim model via black-box adversarial attacks?}

    \begin{enumerate}
        \item \textbf{Exp3.1}: Similar to Exp.1, show the feasibility of model parsing on black-box adversarial attacks (e.g., query-based or transfer attacks).
        \item \textbf{Exp3.1.1}: Universal perturbations.
        \item \textbf{Exp3.2}: Correlation screening to infer unseen model details using existing model attributes and evaluate our inference quality via transfer attacks. 
    \end{enumerate}

      \item \textbf{Experiment cluster 4}: \textbf{What factors could influence model parsing?}

      \begin{enumerate}
          \item \textbf{Exp4.1}: Attack quality? E.g., PGD steps, attack radius, and attack success rates (\textit{i.e.}, generating perturbed examples but not necessarily successful, which can be controlled by robust model vs. standard model, or attack methods)? 
          \item \textbf{Exp4.2}: Victim model robustness? or generalization? Showing model parsing accuracy vs. model's generalization and robustness performance, respectively. 
      \end{enumerate}


      \item \textbf{Experiment cluster 5}: \textbf{What can we learn from model parsing? Better model parsing ability corresponds to what model or attack properties?}

      \begin{enumerate}
      \item \textbf{Exp5.1}: If an attribute is easier to be inferred across datasets/attack methods/model types, does this mean attacks generated from models with the same attributes are easier to transfer? 
       \item \textbf{Exp5.2}: If a specific \textit{attribute combination} is easier to be inferred, does this mean the corresponding model architecture is more vulnerable to attacks (lacks adversarial robustness but with high generalization)? \YY{The top1-precision model architecture is the most vulnerable to adversarial attacks while having the highest generalization. The easiest to be model parsed means the attack has the most prominent model information.}
      \end{enumerate}
\end{enumerate}




    \item \textbf{Conclusion}
\end{enumerate}
